Symplectic Groups, Mapping Class Groups and the Stability of Bounded Cohomology

Mapping class groups satisfy cohomological stability. In this note we show how results by Bestvina and Fujiwara imply that the bounded cohomology does not stabilize, additionally we show that stabily polynomials in the Mumford-Morita-Miller classes are unbounded i.e. their norm tends to infinity as one increases the genus. While the bounded cohomology of the symplectic group does stabilize, we show that it does not stabilize via isometries in degree $2$. In order to establish this we calculate the norm of the signature class in $\mathrm{Sp}_{2h}(\mathbb{R})$ and estimate the norm of the integral signature class.

==> Makefile <==
figuresInput=$(wildcard Figures/*.svg)
figuresOutput=$(figuresInput:.svg=.pdf_tex)
texSources=$(wildcard *.tex */*.tex)

all: pdf

%.pdf_tex: %.svg
	inkscape -z -D --file=$< --export-pdf=$(<:.svg=.pdf) --export-latex && \
	sed -i 's@{\([^{.]*.pdf\)}@{Figures/\1}@' $@

pdf: top.pdf

view: pdf
	evince top.pdf

top.pdf: $(figuresOutput) $(texSources)
	pdflatex top.tex
	biber top.bcf
	pdflatex top.tex
	pdflatex top.tex

spellcheck: $(texSources)
	for file in $^; do aspell --lang=en_US --home-dir=. -t check $$file; done

clean:
	rm -rf top.aux top.log top.out top.blg top.bbl top.pdf Figures/*.pdf Figures/*.pdf_tex

style: $(texSources)
	for file in $^; do sed -i -e's@\s*$$@@' $$file; done

.PHONY: clean style spellcheck

